MOV-Modified-FxLMS algorithm with Variable Penalty Factor in a Practical Power Output Constrained Active Control System

Practical Active Noise Control (ANC) systems typically require a restriction in their maximum output power, to prevent overdriving the loudspeaker and causing system instability. Recently, the minimum output variance filtered-reference least mean square (MOV-FxLMS) algorithm was shown to have optimal control under output constraint with an analytically formulated penalty factor, but it needs offline knowledge of disturbance power and secondary path gain. The constant penalty factor in MOV-FxLMS is also susceptible to variations in disturbance power that could cause output power constraint violations. This paper presents a new variable penalty factor that utilizes the estimated disturbance in the established Modified-FxLMS (MFxLMS) algorithm, resulting in a computationally efficient MOV-MFxLMS algorithm that can adapt to changes in disturbance levels in real-time. Numerical simulation with real noise and plant response showed that the variable penalty factor always manages to meet its maximum power output constraint despite sudden changes in disturbance power, whereas the fixed penalty factor has suffered from a constraint mismatch.

==> Result.tex <==
\section{Numerical Simulation} \label{sec:SimulationResult}
In this section, we conducted a numerical simulation comparison between the proposed variable penalty factor MOV-MFxLMS and other algorithms under different conditions. 
%The output saturation effect is not being considered for all algorithms in this simulation.
\subsection{Convergence path due to a sudden change in disturbance} \label{sec:SimulationResult2Tap}
In this simulation, we compared MOV-MFxLMS with the proposed variable penalty factor, MOV-FxLMS with the predetermined fixed penalty factor, and the conventional FxLMS algorithm when dealing with a sudden varying disturbance. During the simulation, the reference signal was a bandlimited white noise (800--\SI{7200}{\hertz}) with a sudden change in its signal power from $\sigma_x^2 = 0.305$ to $\sigma_x^2 = 0.540$ at the \SI{30}{s} mark. 
% The change in noise power is modeled via a 60-\si{\second} bandlimited white gaussian noise (800--\SI{7200}{\hertz}) with a gain of 0.9 in the first \SI{30}{\second} and 1.2 in next \SI{30}{\second}. 
The optimal penalty factors for the two disturbances are calculated as  $\alpha_1=0.0461$ and $\alpha_2 = 0.3255$, respectively. The sampling rate, step-size, primary and secondary path are set as $F_s = \SI{16}{\kilo\hertz}$, $\mu = 0.0002$, $\mathbf{p} = [1.62 \; 0.41]^\mathrm{T}$ and $\mathbf{s} = [0.03 \; 0.87]^\mathrm{T}$. \fref{fig:Convergence-path} shows the convergence path of the control filter compared between the MOV-MFxLMS, MOV-FxLMS, and the unconstrained FxLMS method. 
% The MFxLMS converges similarly to FxLMS in the simulation as the perfect plant response assumption is used (i.e., $\mathbf{\hat{s}} = \mathbf{s}$). This also indicates that both MOV-MFxLMS and MOV-FxLMS algorithms share the same optimal penalty factor under output constraint (i.e., $\alpha_1$ and $\alpha_2$). While it is true that MFxLMS allows for a larger $\mu$, it is beyond the scope of the current work. 

As shown in \fref{fig:FxLMS}, FxLMS converges to the optimal control filter $\mathbf{w}_{\text{opt}} = [1.62 \; 0.41]^\mathrm{T}$ while ignoring the subjected power constraint of $\rho^2 = 1$, giving the optimal power output for the control signal of $\sigma_{y_\mathrm{o}}^2 = 1.1214$ for the first \SI{30}{\second} noise and $\sigma_{y_\mathrm{o}}^2 = 1.9769$ for the next \SI{30}{\second}. However, MOV-FxLMS presents an interesting case as only one of the two optimal penalty factors was used throughout the simulation. It managed to converge to the first optimal constrained filter in the first \SI{30}{s} when the corresponding $\alpha_1$ was used but failed to converge to the optimal constrained filter in the subsequent \SI{30}{s} with a louder disturbance, violating the power output constraint by having $\sigma_{y_\mathrm{o}}^2 = 1.7630$ shown in \fref{fig:convergence_gamma1}. On the other hand, the fixed penalty factor of $\alpha_2$ yielded a similar observation where convergence occurred only in the corresponding final \SI{30}{s}. Although the constraint was not violated in the first \SI{30}{s} with lower amplitude disturbance, it led to an over-constrained output of $\sigma_{y_\mathrm{o}}^2 = 0.5673$, as shown in \fref{fig:convergence_gamma2}.
%------------------------------------------------------------------------
\begin{figure}[!t] \centering
    \begin{subfigure}{0.49\linewidth}    \centering
    \includegraphics[width=\linewidth]{FxLMS.png} \vspace{-2\baselineskip} 
    \caption{} \label{fig:FxLMS}
    \end{subfigure}
    \begin{subfigure}{0.49\linewidth} \centering
    \includegraphics[width=\linewidth]{MOV-offline_gamma1.png} \vspace{-2\baselineskip}
    \caption{} \label{fig:convergence_gamma1}
    \end{subfigure}
    \begin{subfigure}{0.49\linewidth} \centering
    \includegraphics[width=\linewidth]{MOV-offline_gamma2.png} \vspace{-2\baselineskip}
    \caption{} \label{fig:convergence_gamma2}
    \end{subfigure} 
    \begin{subfigure}{0.49\linewidth} \centering
    \includegraphics[width=\linewidth]{MOV-timeVary_256.png} \vspace{-2\baselineskip} 
    \caption{} \label{fig:convergence_vary}
    \end{subfigure}
    \caption{Two-weight convergence paths of (a) FxLMS, (b)-(c) MOV-FxLMS with optimal penalty factor, and (d) the varying penalty factor MOV-MFxLMS algorithm when dealing with the sudden varying disturbance.} \label{fig:Convergence-path} 
\end{figure}
%------------------------------------------------------------------------
\begin{figure}[t] \centering
    \includegraphics[width=\linewidth]{gamma_2coeff.png}
    \caption{The time history of the variable penalty factor, where the power of disturbance happens to change at $t=\SI{30}{\second}$.} \label{fig:gamma_2coeff} \vspace{-1\baselineskip}
\end{figure}
%------------------------------------------------------------------------

In contrast, the MOV-MFxLMS algorithm with the variable penalty factor and $K=256$ can mitigate this problem. As illustrated in \fref{fig:convergence_vary}, it initially converges to the first optimal constrained filter (red path) and shifts to the second optimal constrained filter (blue path) when the second noise is present, thereby satisfying the power-output requirement for the duration of the simulation. The same phenomena can be observed in \fref{fig:gamma_2coeff}, where the calculated penalty factor changes at $t=\SI{30}{\second}$ due to a change in disturbance power. Due to the moving-average operation from \eref{eqn:Gs_est_new}--\eref{eqn:OptimalPenaltyFactorVary}, the variable penalty factor fluctuates around $\alpha_1$ at the first $30$ seconds and around $\alpha_2$ at the next $30$ seconds. Therefore, this simulation demonstrates that the proposed variable penalty factor MOV-MFxLMS algorithm is capable to achieve optimal constraint control even if the disturbance has a sudden change in amplitude. The same conclusion can be extended to the variation of the primary noise.   
% This can be mitigated when the variable penalty factor MOV-MFxLMS, as described from \sref{sec:EstimationPenalty}, is used with $K=256$. It can be seen from \fref{fig:convergence_vary} that it initially converges to the first optimal constrained filter (red path) and then changes to the second optimal constrained filter (blue path) when the second noise is present, thus satisfying the power output constraint throughout the entire simulation. This can also be observed in \fref{fig:gamma_2coeff} where the calculated penalty factor changes at $t=\SI{30}{\second}$ due to a change in disturbance power. It is also notable that the penalty factor fluctuates between 0 to 0.15 for the first \SI{30}{\second} and between 0.15 to 0.45 for the next \SI{30}{\second} as compared to the fixed optimal penalty factor method since the penalty factor is now a moving average based on the disturbance.   

\subsection{Active control on real noise based on measured paths} 
\label{section:SimulationResultRealMeasurement}
\begin{comment}
\begin{figure}[!t] \centering
    \begin{subfigure}{\linewidth}    \centering
    \includegraphics[width=\linewidth]{anti-noise_time.png}
    \end{subfigure}
    \begin{subfigure}{\linewidth} \centering
    \includegraphics[width=\linewidth]{gamma_time.png}
    \end{subfigure}
    \begin{subfigure}{\linewidth} \centering
    \includegraphics[width=\linewidth]{Gs_time.png}
    \end{subfigure}
    \caption{Broadband noise reduction performance of the MOV-MFxLMS as a function of time by comparing (a): the disturbance and anti-noise signal, (b): the varying and optimal penalty factor when subjected to its power output constraint of $\rho^2 = 1$, and (c): signal power gain through secondary path. $K=1024$ is selected in this simulation.} \label{fig:anti_noise_gamma_time}
\end{figure}

To verify the proposed method in its power output constraint, the proposed varying MOV-MFxLMS algoritm is further used to attenuate a 400--\SI{600}{\hertz} broadband noise with a primary and secondary path measured from an air duct \citep{Shi2021b}. \fref{fig:anti_noise_gamma_time} shows the comparison between the disturbance $d(n)$ and its anti-noise signal through the varying penalty factor $\alpha(n)$, with $K = 1024$, and a fixed optimal penalty factor $\alpha_0$ when the entire signal is known. As the penalty factor changes with time due to its fluctuating moving-average disturbance power and $\hat{G}_s$, it can be shown that there is a difference in the anti-noise signal between the varying and fixed optimal penalty factor. Nevertheless, both varying and constant penalty factor algorithm satisfy the power output constraint, although it is expected for the resulted power output to be not equal to the defined constraint due to its fluctuation. This verifies the moving average estimation method from \eref{eqn:Gs_est_new} and \eref{eqn:OptimalPenaltyFactorVary} which satisfy the output power constraint. 
\end{comment}
To further verify its effectiveness, the proposed varying MOV-MFXLMS algorithm is utilized to attenuate a compounding noise on the primary and secondary path measured from an air duct \citep{Shi2021b}. \fref{fig:changeRealNoise} depicts the error signal and its moving average output power undergoing four distinct noise stages. The first \SI{30}{\second} contains a 400--\SI{600}{\hertz} broadband noise, and a larger amplitude of 400--\SI{600}{\hertz} broadband noise is compounded to the existing noise for the next \SI{30}{\second}. Similarly, a measured construction noise, having a dominant 70--\SI{400}{\hertz} noise, and aircraft flyover noise, having a dominant 400--\SI{3500}{\hertz} noise, is compounded to its previous noise for the 60--\SI{90}{\second} and 90--\SI{120}{\second} time frame respectively. As the acoustic effect on non-linearity varies between different instruments, no output saturation effect shall be considered in this simulation when exceeding the output power constraint.

The FxLMS algorithm has the most noise reduction as shown in \fref{fig:error_changeNoise} while ignoring its output power constraint shown in \fref{fig:power_changeNoise}, especially in the fourth stage where the output power increases tremendously to an approximate peak value of $\sigma_y^2(n) \approx 10$ due to the non-stationary aircraft noise. For MOV-FxLMS with a fixed penalty factor calibrated for the 30--\SI{60}{\second} noise, it can be seen that it only managed to meet the power output constraint during the 30--\SI{60}{\second} period but has exceeded the output constraint during the 60--\SI{90}{\second} and 90--\SI{120}{\second} period due to the additional construction noise and aircraft noise, respectively. In contrast, the power output for the 0--\SI{30}{\second} period has been over-constrained as it showed a lower output power than that of FxLMS and its defined output constraint. This issue can be mitigated by the varying penalty factor MOV-MFxLMS algorithm that managed to maintain the power output constraint for the 30--\SI{120}{\second} period as shown in \fref{fig:power_changeNoise}. It has the same convergence as FxLMS for the first \SI{30}{\second} as the estimated moving averaged disturbance power is less than $K\rho^2\hat{G}_s(n)~(K=1024)$, leading to the calculated penalty factor from \eref{eqn:OptimalPenaltyFactorVary} to be 0. This verifies the moving average estimation method from \eqref{eqn:Gs_est_new} and \eqref{eqn:OptimalPenaltyFactorVary}, which satisfy the output power constraint due to a sudden change in noise type.
\vspace{-1\baselineskip}

\begin{figure}[!t] \centering
    \begin{subfigure}{\linewidth}    \centering
    \includegraphics[width=\linewidth]{error_changeNoise.png} \vspace{-2\baselineskip}
    \caption{} \label{fig:error_changeNoise}
    \end{subfigure} 
    \begin{subfigure}{\linewidth} \centering
    \includegraphics[width=\linewidth]{u_pow_changeNoise.png} \vspace{-2\baselineskip}
    \caption{} \label{fig:power_changeNoise}
    \end{subfigure}
    \caption{The (a): disturbance and error signal, (b): 1024 samples moving average output power $\sigma_y^2(n)$ during control through various adaptive algorithms with $\rho^2 = 0.8.$} \label{fig:changeRealNoise} \vspace{-1\baselineskip}
\end{figure}
